Universal Layout Emulation for Long-Term Database Archival

Research on alternate media technologies, like film, synthetic DNA, and glass, for long-term data archival has received a lot of attention recently due to the media obsolescence issues faced by contemporary storage media like tape, Hard Disk Drives (HDD), and Solid State Disks (SSD). While researchers have developed novel layout and encoding techniques for archiving databases on these new media types, one key question remains unaddressed: How do we ensure that the decoders developed today will be available and executable by a user who is restoring an archived database several decades later in the future, on a computing platform that potentially does not even exist today? In this paper, we make the case for Universal Layout Emulation (ULE), a new approach for future-proof, long-term database archival that advocates archiving decoders together with the data to ensure successful recovery. In order to do so, ULE brings together concepts from Data Management and Digital Preservation communities by using emulation for archiving decoders. In order to show that ULE can be implemented in practice, we present the design and evaluation of Micr'Olonys, an end-to-end long-term database archival system that can be used to archive databases using visual analog media like film, microform, and archival paper.

==> overview.tex <==
\section{System Overview}

Before describing the design of various components of \systemname{} in Section~\ref{sec:design}, we will first present an end-to-end workflow from a user point of view in this section to illustrate the database archival process. 
%Then, we will provide an overview of various components of \systemname{} and how they interact to provide universal  archival of both data and layout algorithms together. 

%\subsection{Usage Overview}

In order to archive a database using \systemname{}, a user has to first extract data from a DBMS. This is done using existing tools, and most current tools produce data as software-independent, user-readable ASCII files. Then, \systemname{} then compresses the data and encodes it to produce a series of images, with each image being a dense array of barcodes. We refer to these barcodes as \emph{emblems} to distinguish them from conventional barcoding and QR-coding techniques, as our emblems are customized for high-density, error-tolerant digital data storage. In addition, \systemname{} also produces a four-page, plain-text description of a simple bootstrap algorithm that a user must implement in the future using any programming language, run time, or computing platform, that will automatically perform data restoration. This bootstrap text and emblems are then physically ``written'' to the analog media via microfilming (for microfilm), shooting (for cinema film), or printing (for archive paper). The media is then archived, possibly for several decades.

At some point in the future, when data needs to be restored, the analog media is retrieved and the emblems are scanned to generate high-resolution images. We make no assumptions about the scanning technology or image format for the images generated. The plain-text pseudocode clearly describes the canonical format into which each image must be converted (a simple, flat 1D-array of pixel intensity values).
%Note that \systemname{} assumes that the media will be readable in the future, albeit with potential errors due to media degradation. This is definitely the case for analog media like microform and cinema reel which have already been used by libraries and archives for decades, are known to last for several hundreds of years, and can be visually inspected and scanned using any light projection technology. 
In the second step, a user implements the bootstrap algorithm using the plain-text pseudocode. It is important to note here that we make no assumptions about the underlying hardware or software environment. Thus, the user can implement the bootstrap algorithm on any host architecture in the future, using any programming language.  After implementing the algorithm, the user executes the program which automatically decodes the emblems in the images and generates the ASCII database archive. The user can then use existing tools to load data back into a future DBMS.



==> related.tex <==
\section{Related Work}
